Reflection in Game-Based Learning: A Survey of Programming Games

Reflection is a critical aspect of the learning process. However, educational games tend to focus on supporting learning concepts rather than supporting reflection. While reflection occurs in educational games, the educational game design and research community can benefit from more knowledge of how to facilitate player reflection through game design. In this paper, we examine educational programming games and analyze how reflection is currently supported. We find that current approaches prioritize accuracy over the individual learning process and often only support reflection post-gameplay. Our analysis identifies common reflective features, and we develop a set of open areas for future work. We discuss these promising directions towards engaging the community in developing more mechanics for reflection in educational games.

==> source/notes.tex <==

% I kind of think this whole paragraph can be removed but if you disagree look at my comment below
%
% This whole paragraph, for me, does not flow together. First  we start broad, which is good, but then we go to some feature related to process displays but then ditch it to go to process prompots. FInally we conclude the paragraph by saying what we will discuss below. Instead, just drop the introduction. We have all that above. It isn't necessary. Then put in your conclusion at the end once you have built up everything else. It will be stronger and read much better. It will also help since you won't have to state so many ideas in a paragraph. 

%Games provide insights for researchers to analyze players learning processes but that insight is not being reflected back two player. 
%Mechanics for assessment must be designed to elicit relevant behaviors that can be observed through the user log and interpreted to reveal the learning process and learner variables 
%What is being reflected back and visualized to the learner is evaluative measures which does not redirect back to the Learners process  -Reflecting back towards the behaviors are summative measures.

%mechanics require the learner to make explicit the steps used for problem solving rather than simply provide the answer to a problem. we're not looking at the steps we are focusing on the summative outcome. 

%Learner process - Discovering unconscious things in the learning domain, about making otherwise implicit things about  behavior explicit. Understanding their misconceptions - faulty thinking


%\textcolor{red}{[How players reflect in a game]}
%James Paul Gee.
    %Reflective practice (rethink cycle) - probe, hypothesize, reprobeProbe the virtual world (involves looking around the current environment, engaging in a certain action, etc)
    
    %Based on reflection during and after probing, the player must form a hypothesis about what something might mean in a usefully situated way (text object, event, etc)
    
    %Reprobes the world with the hypothesis in mind, seeing what effect she gets.The player treats this effect as feedback from the world and accepts or rethinks her original hypothesis.
    
    %Some consider this process to be the basis of expert reflective practice in a complex semiotic domain
    %(Schon )Reflect in action and on the action. Such reflection requires feedback (after reprobe) from the world about the success or failure of your action.
    
%\textcolor{red}{[Why do players want to reflect?]}
%Moon. 
    %Users want to use reflection for: learning the material for further reflection; action or other representation of learning; reflection on the process of learning; critical review; the building of a theory; self-development; decisions or resolutions of uncertainty; empowerment or emancipation; and other outcomes that are unexpected    

%\textcolor{red}{[Why do players need to reflect?]}
%Boud
   % Reflection is an essential tool to allow people to make conscious value choices in their attitudes and practices. It opens opportunities to experience the world and oneself in a fundamentally different way. It is a critical aspect for achieving desired learning outcomes.
%Lin.
    %The aim of teaching students to reflect on their thinking processes is to increase their awareness of their own learning, and to enable them to use that awareness to adapt their thinking in other situations. The power of technology for learning can be greatly enhanced through support for reflection, which helps learners construct the new kinds of knowledge and skills they need in this age of information.
    
   % The "basics" required for success in our increasingly changing society are no longer simply reading, writing and arithmetic, but the ability to think reflectively in order to make sense of information and to adapt learning flexibly to new situations (e.g., Bruer, 1993).
    
    %The ability to reflect upon and oversee one's own state of understanding is closely tied to flexible thinking and problem solving (Bransford & Stein, 1993; Hatano & inagaki, 1992; Salomon & Perkins, 1989; Wineburg, in press)
    %If you are creating a problem solving puzzle game, wouldnt this be a critical aspect to include in your design? If we purely focus on designing exponentially harder puzzles, we can only account for a small audience to even reach those puzzles, potentially resulting in a waste of designers time. Incorporating reflection strategies can aid in progressing player's understanding.


%\textcolor{red}{[Conditions for player reflection]}
%Fleck. What are the right environments for reflection? 

    %1) Allowing for time and flexibility
    %Reflection takes time. Therefore creating or allowing time for reflection is essential. 
    %Reflection can “build up” over levels and be flexible for the user to reflect on a later rather than immediately after a level.

   % 2) Proving structure or guidance to be reflective 
    %Reflection is discussed by many authors as a developmental process, and people can be more reflective with support over time.

   % 3) A reason or encouragement to reflect
    %Reflection is time consuming and not necessarily something that comes naturally to people in all situations, they usually need a reason to reflect or at least encouragement to do so.
   % Efficiency, comparative stats, etc. Start the user off with something to grab onto (efficiency) and prompt other values throughout the experience.

   % 4) Access to material
   % Encouraging review or revisiting of materials or events; using evaluation (for example assessments) to encourage reflection.
    
   % 5) By making the learner's thinking visible, we can change their thinking.


%Sengers. 
    %5) Reflection is effective only when it is immediately folded back into our experiences, actions, identities, and practices, rather than an intellectual practice separate from action.

%\textcolor{red}{[What triggers reflection?]}
%Juul. Failure (or moments of surprise) triggers reflection. 
    %Failure concretely pushes us to search for new strategies and learning opportunities in a game. Failure has the double function of creating in us a feeling of being flawed and forcing us to reconsider our strategies in order to escape that feeling.
    
 Old related work content (in case we need it later)  
% teachers and aar
Prior work in simulated environments for teachers \cite{dieker2017using,hughes2016enhancing,barmaki2018embodiment}, takes a unique approach to reflection by incorporating after-action review (AAR) to structure reflection into their learning experience. Even though this work is not a game experience, this approach allows for active learning and exploration in the virtual setting. Next, they ground the active learning in an integrated AAR process, in which users take part in guided reflection with video tagging software and playback  \cite{dieker2017using,hughes2016enhancing}, audio, and gesture capture \cite{barmaki2018gesturing} and assessments on how the user handled different situations during the session \cite{barmaki2018embodiment}.

%Similarly, this outlines a potential gameplay loop that can be used in educational games. Further, Garris et al., states that reflection needs to be built into the game as a debrief feature. It needs to be part of the design. This idea is further reinforced by literature which has shown that reflection is an integral part of the learners experience \cite{sengers2005reflective,fleck2010reflecting}. This runs alternative to the simplest approach of having learners play a game first and then have a teacher aid in reflection afterwards. 
%An example of this approach can be seen in the work from Emihovich and Miller which had teachers ask reflective questions while students worked through programming tasks with either CAI or Logo \cite{emihovich1988effects}. This, though, runs in parallel to the Schön's work, which found there to reflection-in-action, reflection while taking an action, and reflection-on-action, reflection after an action \cite{Schon1983}. Furthering the concept that education games need to have reflection built into there design. 


%In the context of games, the experimentation of gameplay mechanics affords an individual the opportunity to reconstruct current knowledge of the material in new ways \cite{gee2003video}. Through failure, players can reflect on their current actions \cite{juul2013art,anderson2018failing}, self-correct activities, and build mastery through past experiences \cite{gee2003video}. Failure is an opportunity to bring awareness to unconscious aspects of their routine activity. 
%Once attended to, it can force evaluation and modification of the player's own thinking and problem solving tactics \cite{anderson2018failing, vanlehn1988toward}. Once a player has begun to reflect, they can provide themselves with a variety of motivating reasons to continue, such as, self-development; decisions or resolutions of uncertainty; empowerment or emancipation; and other outcomes that are unexpected \cite{moon2013reflection}.

%Reflection has also been synthesized into a behavioral framework, which addresses levels of reflection that captures the behaviors and activities associated with each level. Fleck et al. creates a reflection framework as a resource for technology design by examining purposes of reflection, conditions for reflection, and then detail how technologies can support these different aspects \cite{fleck2010reflecting}. 

%Another important point when designing for educational games for reflection is that critical reflection needs be part of the design practice. This will help identify blind spots, assumptions, and open up new design spaces \cite{sengers2005reflective}. By designing for reflective opportunities for others, we also need to be reflective as designers to ensure we are not shaping our products based on individual assumptions.

%Reflection is a developmental process \cite{gee2003video,lin1999designing,sengers2005reflective} where people engage to explore experiences which lead to new understandings and appreciations \cite{boud1996promoting}. 
%The process of reflection can bring awareness to the unconscious aspects of one's experience. Once biases and process inefficiencies are exposed, one is able to make a conscious choice for change \cite{sengers2005reflective}.
%It opens opportunities to experience the world and oneself in a fundamentally different way\cite{lin1999designing}.
%Reflection is a critical aspect for achieving any desired learning outcome \cite{lin1999designing,boud1996promoting,gee2003video}. 

%A significant amount of research has been conducted to understand how reflection is part of a larger process for learning \cite{gee2003video,moon2013reflection}, its impact on self-awareness \cite{sengers2005reflective}, learning outcomes \cite{gee2003video,lin1999designing}, and how to design opportunities for reflection in technology \cite{lin1999designing,fleck2010reflecting,sengers2005reflective}.However, designing for reflection in educational games remains an under explored area.
%This research builds off of Donald Schön's studies on professionals revising their practices through trial and error, which is referred to as a "conversation with the system" a process called reflection-in-action. Also,reviewing or analyzing a situation after an event, a process called reflecting-on-action \cite{Schon1983}.  Schön separates reflection opportunities into two areas, during and action and after an action.

Reflection is an an essential tool to allow learners to make conscious value choices in their practices \cite{boud1996promoting} and enables them to adapt their thinking in other situations \cite{lin1999designing,fleck2010reflecting}. 
%Reflection is a process where one can engage in a exploration of experiences which lead to new understandings and appreciations \cite{boud1996promoting}. 
The process of reflection can bring awareness to unconscious aspects of the experience. Once exposed, one is able to make a conscious choice for change \cite{sengers2005reflective}.


% DO WE NEED THIS?
%With a focus on programming games, these games are becoming accepted media for education and training \cite{gee2003video, prensky2003digital,randel1992effectiveness,valls2015exploring}, growing evidence shows that well-designed educational games not only sustain students’ motivation for learning to program but also enhance the learning outcome \cite{barnes2008game2learn,cliburn2006effectiveness,randel1992effectiveness}.Game settings potentially are well-suited to provide reflection a place for both structured play in-action and on-action by bringing unconscious aspects of the gameplay experience to conscious awareness, explicitly making them available for active evaluation to scaffold change.

%As critical as reflection is, learners are not naturally reflective. Reflection is time-consuming and does not necessarily come naturally to people; they usually need a reason to reflect or at least encouragement to do so \cite{fleck2010reflecting}. A clear motivator is failure \cite{juul2013art}. Failure is an opportunity to wake up consciousness from a routine activity, which forces evaluation and modifications of one's thinking and problem solving \cite{anderson2018failing,vanlehn1988toward}.
%Reflection is often triggered by an error or surprise, where someone moves from knowing-in-action, operating within the status quo, to reflection-in-action, puzzling out what to do next or why the status quo has been disrupted \cite{sengers2005reflective,Schon1983}. Reflection in, or on, action often occurs when people are surprised to find their tacit routines failing \cite{juul2013art}. Once started, reflection can provide a variety of motivating reasons to continue to reflect, such as, self-development; decisions or resolutions of uncertainty; empowerment or emancipation; and other outcomes that are unexpected \cite{moon2013reflection}.

----
[other work to possibly consider - creating a game with agent adaptability ]


Towards the design of Intelligent Educational Gaming Systems. This paper focus on these concepts, describing what Intelligent Tutoring Systems (ITS) features can provide to Educational games. We also describe TALENT, a game to teach computer algorithms that incorporates features from ITS. The overall design proposed, is a step towards an Intelligent Educational Gaming System. "Work has been done to incorporate a pedagogical agent.Pedagogical agents can act as virtual tutors, virtual students, or virtual learning companions that can help students in the learning process. It inhabits the educational game environment supporting the learner by giving him appropriate help based on specified teaching strategies and learner’s model. The pedagogical agent is responsible to apply these strategies to learner by intervening in the environment. They support interventions, possible encouraging reflection". \cite{maragos2005towards}

[other work to possibly consider - framework for serious games]
“Reflection should take place within the game without letting the learner step out of the game world, and this can be done by offering reflection activities within the game. Garris et al [5] have stated that the reflection activity can be included within the game by providing a description, an explanation of why this activity is chosen, a discussion of the errors made by the learner, and some corrective suggestions.” This framework focuses on assessments during gameplay. \cite{yusoff2009conceptual}

[other work to possibly consider - Process model for instructional games (motivation and learning)]
Garris et al. discusses learning by doing must be coupled with the opportunity to reflect and abstract relevant information for effective learning to occur and for learners to link
knowledge gained to the real world. They mention a game cycle “doing, reflecting, understanding, and applying” process. \cite{garris2002games}

Literature shows that reflection is not a separate activity but should be incorporated as an integral part of the experience \cite{sengers2005reflective,fleck2010reflecting}. In the case of games, the core gameplay loop should have reflection built into it. Game settings are potentially well-suited to provide reflection a place for both structured play in-action and on-action by bringing unconscious aspects of the gameplay experience to conscious awareness by explicitly making them available for active evaluation to scaffold change.

Lin et al. addresses the importance of reflection and learning as follows "technology, properly designed and used, enables us to realize reflective learning environments that were not previously possible." They identify how technology can be designed to support reflection, and discuss implications for the future design of reflective learning environments. Further, they argue that without appropriate support, students have difficulty engaging in high-level reflective thinking and as a result may limit their ability for knowledge and understanding \cite{lin1999designing}. Lin et al. identified four types of design features that provide scaffolds for reflective thinking that can be integrated into video, the Internet, and large telecommunication systems, which include, 1) Process displays: displaying problem-solving and thinking processes, 2) Process prompts: prompting students' attention to specific aspects of processes while learning is in action, 3) Process models: modeling of experts' thinking processes that are usually tacit so that students can compare and contrast with their own process in action, and 4)  Social discourse: creating community-based discourse to provide multiple perspectives and feedback that can be used for reflection \cite{lin1999designing}. We extend this work to educational games and use these features in our game analysis, we detail this further in section \ref{meth}.

Reflection has also been synthesized into a behavioral framework, which addresses levels of reflection that captures the behaviors and activities associated with each level. Fleck et al. creates a reflection framework as a resource for technology design by examining purposes of reflection, conditions for reflection, and then detail how technologies can support these different aspects \cite{fleck2010reflecting}. 

Additionally, Sengers et al. argues that critical reflection should be a core principle of design practice for identifying blind spots, assumptions and opening new design spaces \cite{sengers2005reflective}. By designing for reflective opportunities for others, we also need to be reflective as designers to ensure we are not shaping our products based on individual assumptions.


Regarding games, recent work has explored how the influence of failure on thinking skills in an educational video game is an integral part of learning and is a trigger for critical reflection \cite{anderson2018failing}.  
The experimentation of gameplay mechanics affords an individual the opportunity to reconstruct current knowledge of the material in new ways \cite{gee2003video}. Through failure, players can reflect on their current actions \cite{juul2013art,anderson2018failing}, self-correct activities, and build mastery through past experiences \cite{gee2003video}.

Prior work in simulated environments for teachers \cite{dieker2017using,hughes2016enhancing,barmaki2018embodiment}, takes a unique approach to reflection by incorporating after-action review (AAR) to structure reflection into their learning experience. Even though this work is not a game experience, this approach allows for active learning and exploration in the virtual setting. Next, they ground the active learning in an integrated AAR process, in which users take part in guided reflection with video tagging software and playback  \cite{dieker2017using,hughes2016enhancing}, audio, and gesture capture \cite{barmaki2018gesturing} and assessments on how the user handled different situations during the session \cite{barmaki2018embodiment}.


Although the synergy between educational games and reflective design for technology has been identified, little work has been done on explicitly integrating reflection into programming games. We surveyed a total of 12 programming games and identified reflective patterns utilizing Lin et. al's four design features, which include 1) Process displays 2) Process prompts 3) Process models 4) and Social discourse \cite{lin1999designing}. We extend this work to educational games and use these features to highlight reflective elements in our game analysis. Additionally, we propose an initial approach to extending reflective work to programming games, focusing on how to improve player reflection toward adaptive thinking.
%The critical aspects of reflection in, and on action, has potential to be integrated within a game structure, by providing a setting to support a balance between gameplay and reflective activities during and after play.

%Further, we aim to develop a understanding of how programming games facilitate reflection to further work in educational programming games. In this paper, we surveyed a total of 12 programming games and identified reflective patterns utilizing Lin et. al's four design features, which include, 1) Process displays: displaying problem-solving and thinking processes, 2) Process prompts: prompting students' attention to specific aspects of processes while learning is in action, 3) Process models: modeling of experts' thinking processes that are usually tacit so that students can compare and contrast with their own process in action, and 4) Social discourse: creating community-based discourse to provide multiple perspectives and feedback that can be used for reflection. \cite{lin1999designing}. We extend this work to educational games and use these features to highlight reflective elements in our game analysis.

%without relying on reflective encouragement from the educator, who may not be present during the game experience, this  . creating a structured reflection experience. which has potential in scaffolding learning outcomes in and outside the classroom, without relying on reflective encouragement on the educator, who may not be present during the game experience. 

%A significant amount of research has been conducted to understand how to incorporate opportunities for reflection in technology design, \cite{lin1999designing,fleck2010reflecting,sengers2005reflective} and their impact on self-awareness \cite{sengers2005reflective} and learning outcomes \cite{gee2003video,lin1999designing,moon2013reflection}.

%Without reflective opportunities designed into the core gameplay loop, programming games run the risk of player automaticity and routine performance \cite{lin1999designing}. Critical reflection provides a means to gain self-awareness and is the first step toward possible progressive change \cite{sengers2005reflective}. Designers have the ability to bringing unconscious aspects of their gameplay experience to conscious awareness, explicitly making them available for active evaluation to scaffold change.

%[discuss what other previous work in games have done in terms of articulating reflection as part of the process]

%Researchers have identified the potential for games to support a balance between gameplay and reflective activities \cite{gee2003video} because reflection is not a separate activity from action but is folded into it as an integral part of experience. By incorporating opportunities for conscious reflection, through failure and other reflective triggers, there is potential in solving this issue of adaptable thinking.


\cite{emihovich1988effects}
The teacher: (1) controlled the elements of the tasks to ensure that students were capable of performing the tasks; 
(2) focused the students' attention on the thinking process necessary for programming the turtle; 
(3) modeled and verbalized mental reasoning strategies when programming the turtle; and 
(4) employed metacomprehension questioning strategies that directed the students' attention to four areas: 
    (a) to reflect on what they previously learned (e.g., "What is - for?"); 
    (b) to evaluate ongoing actions of the turtle in relation to the message the children had given (e.g., "Did the turtle go where you wanted it to go?"); 
    (c) to anticipate future actions of the turtle based on the child's intentions (e.g., "If you do FD 70, where do you think the turtle will move?"); and 
    (d) to consider the necessary sequence of steps to solve each potential problem (e.g., "To make the turtle go up here, what do we need to do first?

old process display

% \textit{Process displays} refers to visualizing a learner's thought process or action paths. This explicitly shows learners what they are doing from a holistic perspective so that they may observe and analyze their reasoning and behaviors \cite{lin1999designing}. For example, a game can track and reveal to the player their moment-to-moment interaction and decisions as they go from level to level. However, none of the games reviewed provided such a granular level of visualization of player actions and decisions. 
% %[what other games do this?] 
% Some games, such as {\em Manufactoria}, {\em SpaceChem}, {\em CodeMonkey}, and {\em CodinGame} provide a aggregate visualizations of players' stats or progress. For example, {\em Manufactoria}, see figure \ref{fig:process display}, displays a tree-like diagram of all the levels inside the game. It visualizes the player's progress by highlighting levels completed and displays level specific content such as the best time and how many parts were used, but only on a successful solution. 

%Does the game display, track, or reveal the player's thought process or action paths?

%progress as it pertains to the specific games elements. For example, highlighting how many parts were used over the course of each level. Or, display component stats during gameplay, such as how many elements are currently in use and how many units have been used in previous attempts. Specifically, Space Chem, provides a comparative view in their visual overview to showcase where you stand among other players solutions. Yet, none track thought process or highlight commonalities between gameplay sessions, in other words, they do not encourage critical thinking and simply provide basic information as it pertains to the game.

%Alternatively, there are cases that the code is highlighted as the solution runs. This could be an example of a process, or the process the player took to complete the problem. These are often simply highlighted as the solution runs. to an action as a player, passively, watches their solution play out. These games, (add), (add), separates the "coding" or active play from the solution running. By testing or submitting their product, the player takes on a passive role and watches their product in action. 

%Reflection must occur on at least two levels to encourage self-monitoring, self-correction, or self-motivation in learning: 1) reflection on a product and its value, 2) reflection on the process by which the product was created \cite{lin1999designing}.


old process prompt
% \textit{Process prompts} refer to elements that prompt or draw the attention of the learner toward evaluating specific actions in their process during or after a problem-solving task. These prompts pose appropriate questions and guide the students in tracking or understanding their process \cite{lin1999designing}. For example, a game can highlight particular player actions during gameplay and to prompt reflection on their actions.
% %Based on our analysis, 9 out of the 12 games used a form of process prompting, those games include:  {\em Blocky:Maze} {\em Cargo-Bot},  {\em Code Combat}, {\em CodeMonkey},  {\em CodinGame}, {\em Human Resource Machine}, {\em LightBolt}, {\em Manufactoria},  and {\em Space Chem}. We can see different forms of prompting, such as 1) prompts on failure where the system suggests ways to fix the solution, 2) during a simulation, the system highlights step-by-step the process the player created, or 3) on request of the players the system prompts examples or hints when they are seeking help.
% Based on our analysis, 9 out of the 12 games used a form of process prompting, those games include:  {\em Blocky:Maze} {\em Cargo-Bot},  {\em Code Combat}, {\em CodeMonkey},  {\em CodinGame}, {\em Human Resource Machine}, {\em LightBolt}, {\em Manufactoria},  and {\em SpaceChem}. We can see different forms of prompting, such as 1) prompts on failure, where the system suggests ways to fix the solution. 2) prompts during a simulation where the system highlights the player's solution step-by-step, or 3) prompts on request of the players where the system displays examples or hints.

% Most commonly, all of these games highlight the execution of code or blocks on a step-by-step basis, which draws the player's attention through the process they have created. These games allow the player to build a solution such as, writing code in \textit{Code Spells}, dragging game components onto a track or board in \textit{Parallel} or \textit{SpaceChem}, or arrange a series of arrows in \textit{Cargo-Bot} or \textit{LightBolt}. When ready, the player submits the solution for execution, and what follows is a visual simulation of the player's solution in action. This method provides meaningful time for the player to reflect on their actions.
% For example, {\em CodeCombat} see figure \ref{fig:process prompt}, a game about writing code to command a hero through battles, highlights what code is being currently used by the hero. This guides the player through a simulation of their solution, and highlights errors in red when they need to improve performance. Additionally, {\em Human Resource Machine}, {\em CodinGame}, {\em Blockly:Maze}, {\em RoboZZle}, and {\em CodeMonkey} had player-driven prompts that provide hints, examples and tutorials of helpful solutions.


%In the case of \textit{CodinGame}, a game about programming puzzles, the prompts are set and do not necessarily provide the guidance the player needs.

%Though, none of the game meet the ideal case described above. Most commonly, games highlight execution of code or blocks on a step-by-step basis which draws the users attention to where the fault in the program likely is. Program execution includes a visual simulation to further aid the player. Essentially, giving guidance to the player on where they need to improve their performance. Code Combat and CodinGame both had prompts that could be selected by users to receive hints that would help users solve the problem. In the case of CodinGame, the prompts are set and do not necessarily provide applicable guidance. 


% Process prompts draw attention or prompts students to evaluate what they did, during or after the problem solving task. They are designs in which the technology poses appropriate questions and guides students in tracking and understanding their own process or actions\cite{lin1999designing}.

% Does the game prompt or guide the player in tracking and understanding their own process?
% Lots of prompting occurs during failure.
%Image example - code combat

%Process prompts are used before, during, or after a problem act to help the user reflect on the problem and their actions. This, in part, helps break up the routine nature of educational programming games by forcing players to think through their own process rather than engaging in routine performance. When used, the system should pose appropriate questions or give applicable guidance to players. These prompts should help students track and understand their own process and actions \cite{lin1999designing}.

    % Cargo-Bot: Maze: highlights, replays on correct, no prompting to specific areas.
    
    % Code Combat: Will provide hints when the user prompts the system.
    
    % Human Resource Machine: There is a boss that may be clicked on that will provide relevant hints. Again these are necessarily questions as the definition from Lin et. al ask for.
    
    % Space Chem: On failure, users are shown what problems in a simulation by highlighting them.
    
    % Manufactoria:  There is a built in prompt where the system will show a simulation that is the worst case scenario rather than any fail case.
    
    % CodinGame: Will provide hints when the user prompts the system. Though this is not an exact fit to the definition as this is not posing relevant questions. Instead it gives useful advice, occasionally with code. Some puzzles come with the solution.
    
    % CodeMonkey: The error messages are more descriptive than most and may help point out where you've gone wrong like, "use turn right instead of turn left". 
    
    

Old process model

% \textit{Process models} refer to comparisons of other expert models who are learning in the same domain. Process modeling shows how another process unfolds so that learners can compare and contrast with their own \cite{lin1999designing}. For example, games can provide a leader board to display the best solutions and provide motivation to try alternate strategies. 
% Based on our analysis, 5 out of 12 games provided comparison opportunities, the games include \textit{Code Spells}, \textit{CodinGame}, \textit{Human Resource Machine}, \textit{RoboZZle} and \textit{SpaceChem}. However, none of these games explicitly incorporate an expert model for players to reference. These games rely on leader boards or averages which are displayed on gameplay assessments to promote comparisons.
% \textit{SpaceChem}, see figure \ref{fig:process_expert}, incorporates a comparative view before and after gameplay. This allows players to see the average score before they engage in the the level and then after which compares their score to the average of other players. 
% Alternatively, some players rely on an informal community to access other player's solutions and reference how they went about solving the problem. 
% For example, in {\em CodinGame}, players are able to view a leader board of alternative solutions which have been ranked via votes from other members of the community. These solutions can also be commented on to spark discussion, share content and provide feedback. Furthermore, players are provided a direct link from the game to the discussions.
% %given access to a forum directly related to the problem at hand and are invited to join a Discord community where they can participate in an active discussion with other members of the community.
% The game {\em Robozzle}, takes a similar approach and has a leader board to highlight best solutions and sorts the content based on solution length. 
%In both games, solutions are meant to be seen after the player has finished solving the problem but this is not enforced or guaranteed.

%Human resource machine displays a assessment and shows average comparisons.
%None of the games analyzed had a built in expert player model that was used to guide and help the player. For example: Code Monkey, built for the classroom, relied on the teachers to full fill this role. In contrast, Human Resource Machine had a built in "boss" that could be clicked on and it would provide players with useful hints to find the correct solution. 

%Other games relied on the community aspect of the game where players could see other experts and how they went about solving the problem. For example, in both CodinGame and RoboZZle, players have access to a social community where solutions can be published and players can refer to them. The problem with these two examples is that the solutions are not built into the gameplay loop. Space Chem, though, allows players to see the weakness in their work after a failed submission. They can then reflect on why the particular area is the problem for the solution.
% "The expert's process is then used as a model for novice students who are learning about the same domain. Process modeling shows how a specific process unfolds and explains why the process occurs as shown (Collins, 1991)"

% Process modeling focuses on the process an expert would use in order to think about or solve specific problems. The expert's process is then used as a model for novice students who are learning about the same domain. Process modeling shows how another specific process unfolds so that students can compare and contrast with their own process in action.

%Process modeling focuses on the process that an expert would use to think about or solve problems. The expert's process is used as a model for students who are learning about the same domain. The process model is meant to show how a specific process unfolds so that students can compare and contrast it with their own process in action. To accomplish this, a model does not have to be explicitly used, though. Instead, a game can also compare players to other players. 

% Does the game compare the player's actions to other player actions?

    % Code Monkey: built for teachers in the classroom to fulfill this role.
    % Human Resource Machine: has a built in "boss" that can be clicked on to provide useful hints to find the solution. 
    % Manufactoria: Transition will find weaknesses in machine to point players to where they need to improve their work.
    % Parallel: Has a built in player model that is not currently exposed. 
    
    % RoboZZle: Due to access to a social community, you are able to access other experts and how they work on the puzzles. You are able to see solution lengths and their comments, if they make them. 
    
    % Space Chem: On failure, players are given access to an expert model that finds weakness in their work. 
    

Old social discourse

% \textit{Social Discourse} refers to the collaborative nature of reflection when a learner seeks feedback from a group to modify their own practice. This can also occur by learners being actively engaged in a discussion with a community to share and gather feedback.
% This can sharpen or guide reflection which is otherwise limited to the learner's own thought process and perspective \cite{lin1999designing}. For example, a game can incorporate a publish feature to share solutions with others playing the game.
% % Reflection can also be social and influenced by a community when an individual seeks feedback from a group and modifies his or her practices based on group feedback. 
% % Feedback from the group can sharpen or guide reflection as a means to support their individual process, which was otherwise limited on his or her own thought process \cite{lin1999designing}.
% %Reflection can be social and influenced by a community. An individual can seek feedback from a group and modify their practices based on, hopefully, helpful responses. This can also occur by players being actively engaged in a discussion that may not be directly related to themselves but instead to the problem at hand. This can sharpen or guide reflection as a means to support their individual process, which is otherwise limited to their own thought process and perspective \cite{lin1999designing}.
% In our analysis, 5  out of 12 games provided a social discourse component, those games include \textit{CodeCombat}, \textit{Code Spells}, \textit{CodinGame}, \textit{RoboZZle}, and \textit{SpaceChem}.  The only game that explicitly incorporated community into the game and did not treat it as a separate component was \textit{Code Spells}. \textit{Code Spells},  see figure  \ref{fig:social_discourse}, is a game about coding spells and allows the player to browse a library of other published spells for reference or directly edit in their own gameplay. Spells can also be published to the community.
% Another game that promotes a community feature is in {\em CodinGame}, players are able to share and rank solutions for the leader board. These solutions can also be commented on to spark discussion, share content and provide feedback.
% Alternatively, in the games \textit{SpaceChem} and \textit{CodeCombat} players can access an informal community where they can participate in a public form to ask and answer questions. %Aside from Code Spells, is that these games donot build in a social component that the solutions are not built into the gameplay loop.

% Although \textit{Code Monkey} is not included in the 5 games above, it was built to be used inside a classroom as a way to handle the social component. It provided teachers with references to helpful game solutions to use during their lectures and a portal to see  their students solutions and analyze how their progress.

%All four include a public forum where players can ask and answer questions. Space Chem and Code Combat include a leaderboard, and CodinGame has solutions that can be up and down voted by the community. Code Spells allows for users to publish their work that can be seen and referenced by others. Code Combat had the additional feature where players can group up together to create a peer group to work and discuss problems together. SpaceChem had the additional feature where player's can  find "expert" solutions to puzzles through the leader board.
%For example, in both CodinGame and RoboZZle, players have access to a social community where solutions can be published and players can refer to them. The problem with these two examples is that the solutions are not built into the gameplay loop. SpaceChem, though, allows players to see the weakness in their work after a failed submission. They can then reflect on why the particular area is the problem for the solution.


Old Intro
%\section{ Old Intro}
%OLD INTRO
%Reflection is an an essential tool to allow learners to make conscious value choices in their practices [6] and enable them to adapt their thinking in other situations [11,16]. 
%The process of reflection can bring awareness to unconscious aspects of the experience. Once exposed, one is able to make a conscious choice for change [21].Reflection is a critical aspect of any learning process [6,13,16]. The ability to reflect upon and oversee one’s own state of understanding is closely tied to flexible thinking and problem solving [7,16],essential qualities designers aim to encourage in educational games.While educational games can have positive impacts on learning[13], the focus remains on supporting learning concepts through gameplay rather than designing opportunities for reflection. To improve learning outcomes and performance, we must look toward reflection as a critical piece of the overall design [11,13,16,21].
%Often, educational games leave reflection to post-gameplay assessments or debriefs of how a player did after gameplay \cite{garris2002games,yusoff2009conceptual}, such as a description of events that occurred in the game. However, literature suggests that this is not nearly enough \cite{sengers2005reflective,fleck2010reflecting,lin1999designing}. 

%Designers should not treat reflection as a separate activity from action but, instead, fold it into the experience as an essential part of the design \cite{sengers2005reflective} and support multiple ways to facilitate reflection \cite{fleck2006supporting}. For example, a deeper level of reflection can be reached if designers encourage comparisons between multiple perspectives \cite{fleck2006supporting,lin1999designing}. This technique helps learners notice new things about themselves or others that they might otherwise overlook \cite{bransford1993ideal}, making the learners own thinking an object for reflection \cite{lin1999designing}.
%Further, literature states that learners are not naturally reflective. Reflection is time-consuming and does not necessarily come naturally to people; they usually need a reason to reflect or at least encouragement to do so \cite{fleck2010reflecting}.
%More work is needed to address better opportunities for reflection in educational games to extend the learning process.

%Assessments are viewed as opportunities for students to reflect on content as welt as on their learning strategies. Assessments also enable students to determine ways of improving their learning strategies, as necessary.
%Often, these games are not designed for the classroom and when it is, reflection is left for the teacher and student to initiate after gameplay. 
%Often, these games are not designed for the classroom but, when they are, reflection is left for the teacher and student post-gameplay. 
%However, some educational games display base-level assessments of gameplay performance. and often they focus on  

%While teachers are the single most important factor to influence student learning and academic outcomes, aside from the students themselves \cite{darling2003keeping}, designers have an opportunity to learn from reflective teaching practices \cite{dieker2017using} and consider approaches in game development.

%Unfortunately, literature suggests that learners are not naturally reflective. Reflection is time-consuming and does not necessarily come naturally to people; they usually need a reason to reflect or at least encouragement to do so \cite{fleck2010reflecting}. Many authors discuss reflection as a developmental process \cite{gee2003video,lin1999designing,sengers2005reflective}, and people can be more reflective with support over time. Without reflective guidance, self-awareness and adaptive thinking are at risk of being lost to routine problem-solving, missing opportunities to mold active learning into critical 'meta' understanding \cite{gee2003video} for use in real life \cite{sengers2005reflective}.

%In this paper, we aim to develop a further understanding of how to design reflective opportunities in educational games. We narrow our focus to a sub-genre of this domain, programming games. Programming games are especially well-suited to examine reflection since reflection is more likely to be invoked in learning environments in which complex problems are embedded, because of increased demand for conscious decision making and questioning \cite{lin1999designing}.
%Therefore, we aim to better understand how programming games currently facilitate reflection. 

%We surveyed a total of 12 programming games utilizing Lin et al.'s \cite{lin1999designing} four reflective design features, which include, 1) Process displays: displaying problem-solving and thinking processes, 2) Process prompts: prompting students' attention to specific aspects of processes, 3) Process models: modeling of experts' thinking processes so that students can compare and contrast with their own process, and 4) Social discourse: creating community-based discourse to provide multiple perspectives and feedback that can be used for reflection. We use these features to identify reflective elements that are used in each game and discuss the commonalities that occur.
%Furthermore, we propose an initial approach to improve player reflection in educational games.


Section 5 notes
 
%Local issue

%Debriefs don’t provide value outside the immediate context.  Cool I got 4 starts but what did I do to get those? What does 3 star look like? Cargo not or Human Resources

%Prompt issue - How can I improve  or better look at what I’m doing

%External issue - most social discussions are outside of the game. There could be more work in exploring this together.

%Reflection in action is avoided but does provide some ui to look at

 %Revisiting with Explanation Description including justification or reasons for action or interpretation, but in a reportive or descriptive way. No alternate explanations explored, limited analysis and no change of perspective
 
 %Exploring Relationships A different level of thinking about. Looking for relationships between pieces of experience or knowledge, evidence of cycles of interpreting and questioning, consideration of different explanations, hypothesis and other points of view.


%To the best of our knowledge, we have not found a direct effort to incorporate reflective design features into educational games. We believe that incorporating elements of existing design features proposed by Lin et al. \cite{lin1999designing} and structured reflection experiences, such as After-Action-Review (AAR), used by simulated environments for teachers \cite{dieker2017using,hughes2016enhancing,barmaki2018embodiment} can be a useful starting point for improving reflection in educational games.Below we offer our design considerations to other designers interested in exploring this space.

old related works

%\section{Old Related Works}
%Reflection has been an important focus for many researchers; however, most of the research work in this area idles in theory, for example, current work synthesizes literature into frameworks \cite{fleck2010reflecting,yusoff2009conceptual}, design features \cite{lin1999designing,sengers2005reflective}, and other process models \cite{garris2002games} with a spotlight on learning environments and technology design. There is a significant need to push these theories into the realm of practice because as games are becoming accepted media for education and training \cite{gee2003video, prensky2003digital,randel1992effectiveness,valls2015exploring}, growing evidence shows that well-designed educational games not only sustain students’ motivation but also enhance the learning outcomes \cite{barnes2008game2learn,cliburn2006effectiveness,randel1992effectiveness}. With this in mind, designing for reflection in educational games is an essential next step to advance not only games, but enables us to realize a potential new setting for reflective learning environments.
%Yet, this s remains an under explored area.
%however, some designers talk about "thinking meta" Skill → strategy. John Beck and Mitchell Wade - The fact that you take a step back from the immediate situation, analysing the choices and the odds, and find the right strategy. This process allows you to move from skill to strategy. You cant do this without reflection. "Take a step back = reflection. This word is so common often, its overlooked even by the most vocal about educational game design.
%Previous work has been conducted to understand how reflection is part of a much larger process for learning and development \cite{gee2003video,moon2013reflection, Schon1983}, its impact on self-awareness \cite{sengers2005reflective}, and learning outcomes \cite{gee2003video,lin1999designing}. Additional work has been done regarding design features and how technology can be created to support reflection in learning environments \cite{lin1999designing,fleck2010reflecting}. In this paper, we aim to use this design theory to further understand how to design reflective opportunities in educational games.
%In this paper, we aim to use this design theory into programming games to further understand how to design reflective opportunities in educational games.


%a significant amount of research has been conducted to understand reflection impacts learning \cite{gee2003video,moon2013reflection}, self-awareness \cite{sengers2005reflective}, and learning outcomes \cite{gee2003video,lin1999designing}. Additional work has been done to find the best ways to design opportunities for reflection in technology \cite{lin1999designing,fleck2010reflecting,sengers2005reflective}. However, designing for reflection in educational games remains an under explored area.
%We find various attempts to address reflection in games \cite{yusoff2009conceptual, garris2002games,anderson2018failing}, simulated environments for teachers \cite{dieker2017using,hughes2016enhancing,barmaki2018embodiment} and educational technologies \cite{lin1999designing,fleck2010reflecting}, however we have not found existing work that addresses reflective \textit{design} for educational games.


%Regarding games, Yusoff et al. designed a conceptual framework for serious games on the basis of nine different principles, with reflection being one \cite{yusoff2009conceptual}. They based this reflection principle on the basis of previous work by Garris et al. in which they discuss using a debrief, a review and analysis of events that occurred in the game, to provide a link between the game cycle and learning outcomes. Garris et al. argue that learning by doing must be coupled with the opportunity to reflect, a "doing, reflecting, understanding, and applying" process \cite{garris2002games}. 
%Yusoff et al. highlighted this work in their framework by creating a separate reflection activity that provides players a description, an explanation of why this activity is chosen, a discussion of the errors made by the learner, and some corrective suggestions after gameplay.  
%However, the literature suggests that reflection is time-consuming, and learners are not naturally reflective on their own, learners need to be supported with time and structured guidance to reflect \cite{fleck2010reflecting}.

%Even though this research does not focus on games, simulated learning environments for teachers extend a similar debriefing approach to encourage reflection \cite{dieker2017using,hughes2016enhancing,barmaki2018embodiment}. They incorporate after-action review (AAR) to structure reflective guidance into their learning experience.
%AAR provides users \textit{time} to reflect and \textit{guidance} with video tagging software and playback  \cite{dieker2017using,hughes2016enhancing}, audio, and gesture capture \cite{barmaki2018gesturing} and assessments on how the user handled different situations during the session \cite{barmaki2018embodiment}. In other words, this reflection activity is designed for the user to take on a more active role in reflection. Since learners can be more reflective with support over time \cite{fleck2010reflecting}, they often need encouragement to draw attention to critical areas, such a debriefing or AAR content. One of those motivators is failure \cite{juul2013art, anderson2018failing}.

%Recent work has explored how the influence of failure in an educational game is an integral part of learning and is a natural trigger for reflection \cite{anderson2018failing}. 
%When players experiment or fail with gameplay mechanics, it affords them the opportunity to reconstruct current knowledge of the material in new ways \cite{gee2003video}. Through failure, players can reflect on their current actions \cite{juul2013art,anderson2018failing}, self-correct activities, and build mastery through past experiences \cite{gee2003video}.

%Finally, Lin et al. discuss how technology can be designed to support reflection and uses examples of how programs and learning environments can incorporate design features to scaffold  reflective thinking \cite{lin1999designing}. The four design features are as follows:
%\begin{enumerate}
   % \item Process displays: displaying problem-solving and thinking processes.
    %\item Process prompts: prompting students' attention to specific aspects of processes while learning is in action.
    %\item Process models: modeling of experts' thinking processes that are usually tacit so that students can compare and contrast with their own process in action.
   % \item Social discourse: creating community-based discourse to provide multiple perspectives and feedback that can be used for reflection.
%\end{enumerate}
%Further, Lin et al. points out that technology provides a new set of opportunities for reflection, "technology, properly designed and used, enables us to realize reflective learning environments that were not previously possible." Therefore, games are a clear next step to advance our understanding of reflective thinking and design.
%Additionally, they argue that without these appropriate supports, students that have difficult in engaging in reflective thinking may limit their own ability to obtain knowledge and understanding.  
%Using these four design features in the context of educational games is a step toward identifying what features are currently occurring and provides a direction on where they could go next. 

%The synergy between educational games and reflective design is clear, yet little work has been done on explicitly integrating reflection into educational games. In this paper, we focus on programming games because they are especially well-suited to examine reflection since reflection is more likely to be invoked in learning environments in which complex problems are embedded, because of increased demand for conscious decision making and questioning \cite{lin1999designing}.
%First,  we aim to better understand how programming games currently facilitate reflection. 
%Secondly, we surveyed a total of 12 programming games utilizing Lin et al.'s four reflective design features to highlight what reflective elements are being used and the commonalities that occur.
%Finally, from our analysis we propose an initial approach to improve player reflection in educational games.

Definitions

(1) Process displays: They are displays that visualize problem-solving and thinking processes. This feature reflects back to students the process they have engaged in as tracked and analyzed by the program. 
For example, Geometry Tutor was designed to teach students geometry. The program used process displays to trace, record, and visually display students' thought and action paths in inspectable tree diagrams.
(2) Process prompts: They are designs, such as a pop-ups, windows, or pages in an digital interface that pose appropriate questions and guide students in tracking and understanding their own process. 
%We use two examples to address how process prompts can be used to encourage reflection by directly asking students questions or indirectly by helping students generate their own questions.
For a direct example,  in the Isopod Simulation Program, uses process prompts to ask students questions and to encourage students to explain their thought process through a pop up window with text.
For an indirect example, CIR-CSIM-Tutor program uses process prompts to aid student reflection on error. This window displays content specific tasks and assesses the student's work against the given criteria. 
(3)Process models: These displays showcase an experts' thinking processes so students can compare and contrast with their own process. 
For example, ASK Jasper, a computer-based learning environment, teaches students basic geometry through designing a swing set. Students can compare and contrast their own designs and reflect on the design process of an expert. 
(4) Social discourse: This is a space for community-based discussion where students can examine multiple perspectives and receive feedback on their own process that can be used for reflection. 
For example, CSILE is a program for students to collaborate. In this program students can discuss questions and collaborate to understanding a problem.
